$Z\gamma$ production in association with two jets at next-to-leading order QCD

Next-to-leading order QCD corrections to the QCD-induced $pp \rightarrow l^+l^- \gamma j j +X$ and $pp \rightarrow \bar{\nu}_l \nu_l \gamma jj+X$ processes are presented. The latter is used to find an optimal cut to reduce the contribution of radiative photon emission off the charged leptons in the first channel. As expected, the scale uncertainties are significantly reduced at NLO and the QCD corrections are phase space dependent and important for precise measurements at the LHC.

==> Makefile <==
MAIN_SRC = QCDZA
BM = --interaction=batchmode

ARCHFLG  = $(shell if test `uname -m` == "x86_64" || \
	test `uname -m` == "i686"; then echo "ghostview"; \
	else echo "preview"; fi) 

MAIN:
		latex $(MAIN_SRC).tex
		bibtex $(MAIN_SRC)
		latex $(MAIN_SRC).tex
		latex $(MAIN_SRC).tex
		dvips $(MAIN_SRC).dvi
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf

diff:
	latexdiff-vc --force --svn -r $(r) $(MAIN_SRC).tex
	latex  $(BM) $(MAIN_SRC)-diff$(r).tex || :
	bibtex $(MAIN_SRC)-diff$(r)
	latex  $(BM) $(MAIN_SRC)-diff$(r).tex || :
	latex  $(BM) $(MAIN_SRC)-diff$(r).tex || :
	dvips  $(MAIN_SRC)-diff$(r).dvi
	ps2pdf $(MAIN_SRC)-diff$(r).ps $(MAIN_SRC)-diff$(r).pdf

preview:
	 	$(MAKE)
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
		open -a Preview $(MAIN_SRC).pdf

ghostview: 
	 	$(MAKE)
		gv -antialias $(MAIN_SRC).ps &

gv:
		$(MAKE) $(ARCHFLG)

pdf: 
		$(MAKE) 
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
		zip $(MAIN_SRC)pdf.zip $(MAIN_SRC).pdf

feyn:


tar:	         
	        $(MAKE)  
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
	        tar cvf $(MAIN_SRC).tar $(MAIN_SRC).pdf $(MAIN_SRC).tex Makefile distributions

clean:
		rm -f *.log *.1 *.t1 $(MAIN_SRC).pdf $(MAIN_SRC).ps *.aux *.dvi *~
		rm -f *.toc *.lof $(MAIN_SRC).tar.gz *.end

